On the Diversity of Analogy Making in Large Language Models

Large Language Models (LLMs) have demonstrated remarkable potential for analogy making, a core cognitive capability that drives novelty and creativity. While prior research has extensively investigated the applications and underlying mechanisms of LLM-based analogy making, its output diversity remains largely unexplored, despite being essential for broadening cross-domain connections and fostering scientific innovation. In this work, we present a comprehensive evaluation of analogy diversity across ten state-of-the-art open- and closed-source LLMs. Our findings highlight a concerning issue of domain homogeneity, a prevalent tendency for LLMs to generate analogies from a narrow set of target domains, limiting both inter-query and intra-model diversity. Furthermore, our analysis reveals a fundamental trade-off in existing LLM diversity-enhancement methods: increasing output diversity often comes at the expense of output quality. Finally, our causal analysis of LLM information flow reveals substantial differences in the model-sensitive regions governing analogy diversity across LLMs, suggesting a potential mechanism for the observed diversity-quality trade-off. To our knowledge, this is among the first studies to systematically investigate output diversity in LLM-based analogy making.

==> Texts/texts_old/s4_solution_old.tex <==
\section{Diversity-Quality Tradeoff in Analogy Making}
\label{sec:solution}

% --------- VERSION 1 -----------


% To address the issue of domain homogeneity, we introduce #NAME, a novel, training-free framework that relies solely on the inherent ability of LLMs to promote analogy-making diversity. Different from several recent studies have explored the direct exchange of hidden-state representations across models\cite{!}, our work is primarily inspired by Patchscopes \cite{ghandeharioun2024patchscopes}, which demonstrates the ability of LLMs to interpret hidden states for improved mechanistic interpretability. In our case, DivGuide goes beyond explanation: we show that LLMs are not only capable of extracting interpretable information from hidden representations, but can also actively edit them, with the model itself serving as an effective guide for the editing process. DivGuide is composed of three steps under the autoregressive generation setup: 
% \daniel{Henry, describing this topics is a good place to describe the exchange of hidden state} 
% \textbf{(1) Hidden State Extraction} collecting the intermediate computation of hidden states from a certain model layer that needs editing, \textbf{(2) Guided Edit} taking the generalization ability of the model itself to edit and guide the hidden states under the instruction of the guide prompt to promote the exchange of hidden states, and \textbf{(3) Patched Generation} replaces the edited hidden states back to the model, continuing the forward pass to generate the next token. Algorithm 1 describes the complete process of DivGuide. 

%their goal often focus on either extracting interpretable information \cite{ghandeharioun2024patchscopes}
% SAE, early-decoding, logit lens
%or steering model behavior under a black-box setting \cite{SteeringACL26}.
% looped transformer + learning based approach

% --------- VERSION 2 -----------

To address domain homogeneity, we introduce \newMethod, a novel, training-free framework that leverages the inherent reasoning capabilities of LLMs to guide the modification of hidden-state representations at inference time of target domain, thereby promoting diversity in output generation for analogy-making.  While prior work has explored hidden-state replacement either for extracting interpretable representations \cite{ghandeharioun2024patchscopes} or for steering model behavior in black-box settings \cite{SteeringACL26}, these directions have remained largely independent. Our work is among the first to unify these perspectives within a single framework: we show that these exchanges can be actively understood and modified by the model \textit{itself} to guide its behavior afterwards during autoregressive generation.

The main hypothesis underlying \newMethod is that LLMs are inherently optimized to generate precise and coherent responses, often at the expense of novelty. Thus show that during the autoregressive generation process, hidden-state representations can be strategically guided to induce more diverse semantic representations, particularly when generating the target domain of an analogy. In practice,  \newMethod is composed of three components: 
\textbf{(1) Hidden State Extraction,} selectively collecting the intermediate computation of hidden states from a certain model layer that needs editing, \textbf{(2) Guided Edit,} taking the generalization ability of the model itself to edit and guide the hidden states under the instruction of the guide prompt to promote the exchange of hidden states, and \textbf{(3) Patched Generation,} replaces the edited hidden states back to the model, continuing the forward pass to generate the next token. Algorithm 1 below describes the complete process of \newMethod. 

\paragraph{Notations for Algorithm 1.} \hspace{-2mm} Let $P_{\theta}$ denote the autoregressive Large Language Model (LLM) with frozen parameters $\theta$. Let $x_{src}, x_{guide}$ denote the input sequences that are being processed by $P_{\theta}$. Let $N$ denote the maximum number of tokens that $P_{\theta}$ can generate. Let $x_t$ denote the distribution of the next token within the model's output dictionary $\mathcal{V}$ at time step $t$. Let $h$ denote the intermediate computations from $x$ in $P_{\theta}$. Let $l$ denote the specific layer index where editing of $h$ is applied. Let $\alpha$ be the steering weight. Let $\mu$ be the average embedding scale normalized from the sequences and $\mathcal{H}(\mathbf{x}_t)$ the entropy function of token $\mathcal{H}(\mathbf{x}_t)$.



% -------ALGO 1-----------

% Define a custom column type for the algorithm steps to handle wrapping and alignment
\newcolumntype{Y}{>{\RaggedRight\arraybackslash}X}

\begin{table}[ht]
% \centering
% \caption{Core HiddenPatch Algorithm (Translator \& Cross-model Disabled)}

\small
\renewcommand{\arraystretch}{1.3}
% Use \columnwidth instead of \textwidth for single-column fit
\begin{tabularx}{\columnwidth}{l Y}
\toprule
\multicolumn{2}{l}{\textbf{Algorithm 1} DivGuide for Generation Diversity} \\ 
\midrule
1 & \textbf{Input:} Model $P_{\theta}$, Input sequence $x_{src}$, Guide sequence $x_{guide}$, Edit layer $l$, Output length $N$, Steering weight $\alpha$, Entropy threshold $\tau$, Average embedding scale $\mu$ \\ \addlinespace
2 & \textbf{Output:} Generation sequence $X_t$ \\ \addlinespace
% 3 & \textbf{Initialize:} \\
%   & \quad $x_{<t} \gets \text{Tokenize}(x_{src})$ \\
%   & \quad $x_{guide} \gets \text{Tokenize}(P_{guide})$ \\ \addlinespace
% Using a loop counter or consistent numbering
3 & \textbf{for} $t = 1$ \textbf{to} $N$ \textbf{do}: \\ 
4 & \quad $x_{t} \sim P_{\theta}( \cdot |x{<t})$ \\
5 & \quad \textbf{if} $\mathcal{H}(x_t) \geq \tau$ \textbf{and} $is\_domain(x_{<t})$: \\
% 5 & \quad \quad $h_{src}^{(L)} \gets M(X_t).hidden[L]$ \\
6 & \quad \quad $h_{src}^{(l)} \gets  h \cdot \frac{\mu_{guide}}{||h||_2} \mid \forall h \in h_{src}^{(l)}$ \\
7 & \quad \quad $x_{guide}' \gets [x_{prefix}; h_{src}^{(l)}; x_{suffix}]$ \\
7 & \quad \quad $x_{guide}' \gets [x_{guide} + h_{src}^{(l)}]$ \\
8 & \quad \quad $h_{edit}^{(l)} \gets P_{\theta}(x_{guide}')$ \\
8b & \quad \quad $h_{edit}^{(l)} \gets P_{\theta}([x_{guide} + h_{src}^{(l)}])$ \\
% 9 & \quad $H_{edit} \gets H_{edit}[\text{indices of } H_{scaled}^{(L)}]$ \\
9 & \quad \quad $h_{edit}^{(l)} \gets h \cdot \frac{\mu_{src}}{||h||_2} \mid \forall h \in h_{edit}^{(l)}$\\
% 11 & \quad $H_{edit}^{(L)} \gets M(H_{edit}).hidden[L]$ \textit{// Re-encode} \\
% 12 & \quad $\alpha_t \gets \alpha \cdot (0.2 + 0.8 \cdot \cos(\frac{\pi \cdot (t-1)}{2 \cdot N}))$ \\
10 & \quad \quad $h^{(l)} \gets h_{src}^{(l)} + \alpha_t \cdot (h_{edit}^{(l)} - h_{src}^{(l)})$ \\
11 & \quad \quad $x_{t} \sim P_{\theta}(\cdot|h^{(l)})$ \\
12 & \quad $X_t \gets [x_{<t}; softmax(x_t)]$ \\
13 & \textbf{end for} \\
\bottomrule
\end{tabularx}
% \caption{}
\label{tab:algo}
\end{table}


% ------------------


% \daniel{We need to provide some definitions, the letter of source and guided model. }





% --------- VERSION 1 -----------

% Given $M$ and input source prompt $P_{src}$, $M$ first encode $P_{src}$ into the sequential embeddings $X_t$ and perform forward pass through the first $L-1$ layers. Then at layer $L$, the hidden states $H_{src}^{(L)}$ are extracted and normalized with respect to the average embedding scale $\mu_{embed}$, which is reflected in line 5-6 in Algorithm 1. The average norm of the sequence in the embedding space $\mu_{embed}$ is calculated as follows:
% \begin{equation}
%     \mu_{embed} = \frac{1}{|X_t|}\sum_{h_i \in X_t} ||h_i||_2
% \end{equation}
% where $|X_t|$ is the length of the generation sequence. The re-scale step ensures that $H_{src}^{(L)}$ is aligned with relative scales within the embedding space, as well as keeping it recognizable to the guide model in the guided edit step so that it prevents potential hidden state collapse in the forward computation.


% --------- VERSION 2 -----------

\daniel{I dont think this is extraction, seems more as whether activating or not the method.}

\paragraph{Hidden State Extraction.} \hspace{-2mm} At each generation time step $t$, $P_{\theta}$ first do a complete forward pass to obtain the next token distribution $x_t$ without any perturbations (Line 4 in Algorithm 1). Then, the entropy of $x_t$ is calculated using Equation\ref{eq:entropy}, reflecting the output uncertainty of $P_{\theta}$. To ensure that we are only guiding the selection of \textbf{domain tokens} during analogy-making, we define an additional function $f:is\_domain()$. We utilize a verifier $f$ (in our case, $f$ is the model itself) that takes the sequence $x_{<t}$ generated so far and decide whether the next token is indeed processing the selection of domain in analogy making. The entropy calculation and the verifier decision is chained together using and gate logic. In other words, only token distributions $x_t$ with both an entropy higher than the threshold $\tau$ and it being verified as a the domain token will it be extracted (Line 5 in Algorithm 1). To further validate the association between domain token generation and its entropy, we include an additional study that records the interplay between these two conditions in Appendix \ref{}.

\begin{equation}
    \mathcal{H}(\mathbf{x}_t) = -\sum_{v \in \mathcal{V}} p_\theta(v \mid x_{<t}) \log p_\theta(v \mid x_{<t})
    \label{eq:entropy}
\end{equation}



% --------- VERSION 1 -----------

% \paragraph{Guided Edit.} \hspace{-2mm} In this step, we follow the existing architecture of teacher-student framework \cite{!}, an effective approach to steer LLM output behaviors. However, different from the typical setting of using a more capable model as the teacher model (i.e. models with larger parameter sizes or models with stronger reasoning capabilities), DivGuide replaces the teacher model with the student model \textbf{itself}. Specifically, we first initialize the guide prompt in natural language $P_{guide}$ into embeddings $E_{guide}$, which consists of two portions including $[E_{prefix}, E_{suffix}]$. Second, we assemble $H_{src}^{(L)}$ with $E_{guide}$ and form a concatenated $E_{guide}'$, which is then fed into the teacher model $M$ and follows a similar procedure described in hidden state extraction, including the re-scale and re-encode steps to obtain the edited hidden state $H_{edit}^{(L)}$. The process is showcased between line 7-11 in Algorithm 1. Setting teacher model equivalent to student model has the benefit of rendering $H_{src}^{(L)}$ recognizable and understandable by the teacher model. Since both models follow identical hidden state manifolds during forward pass, this further allows for more efficient information exchange between hidden states. \henry{We don't have evidence here to support our claim.} 


\paragraph{Guided Edit.} \hspace{-2mm} Once we identify the domain tokens being generated using the joint decision outcomes from hidden state extraction above, we further leverage the generalization ability of LLM \textit{itself} and steer the output behavior in order to promote analogy-making diversity. Intuitively, the editing step is controlled by a separate prompt encoded as the guide sequence $x_{guide}$ in conjunction with $x_t$ that is being edited. We introduce three sub-steps that facilitates the guided editing step which is detailed below. 

First, the identified hidden sequence $h_{src}^{(l)}$ extracted from layer index $l$ is rescaled with respect to the averaged second norm of embedding sequence of $x_{guide}$ (Line 6 in Algorithm 1). This step aims to adapt $h_{src}^{(l)}$ in order to acclimate to the embedding subspace within $x_{guide}$ and to avoid potential collapse during forward pass, as is observed in \citet{}. Second, the rescaled $h_{src}^{(l)}$ is assembled with $x_{guide}$ within the embedding space of $P_{\theta}$ to conduct a separate forward pass and obtain the edited hidden sequence $h_{edit}^{(l)}$ (Lines 7 and 8). Finally, $h_{edit}^{(l)}$ is normalized with respect to the averaged second norm of embedding sequence of $h_{src}^{(l)}$ (Line 9). We note that only indices \daniel{which indices??} that is associated with the original $h_{src}^{(l)}$ is retained in order to maintain a targeted editing of $h_{src}^{(l)}$. Detailed prompts of $x_{src}, x_{guide}$ are included in Appendix \ref{}.




% Specifically, the guide embeddings $E_{guide}$ are assembled by concatenating a prefix $E_{prefix}$, the scaled hidden state $H_{scaled}$, and a suffix $E_{suffix}$. The model $M$ then processes $E_{guide}$ to extract the final layer's hidden states, $H_{edit\_last}$, which represent the model's internal interpretation of the source features under the guidance of the prompt. To maintain numerical consistency, the specific indices corresponding to the source features, $H_{edit\_ct}$, are re-scaled and passed through the model’s first $L$ layers again. This re-encoding process produces the final edited state $H_{edited\_L}$, mapped back into the representation space of the original edit layer $L$.

\paragraph{Patched Generation.} \hspace{-2mm}  The final step involves interpolating the edited features back into the primary generation residual stream. We calculate the difference between the edited state $h_{edit}^{(l)}$ and the original state $h_{src}^{(l)}$, scaling this delta by a dynamic steering weight $\alpha_t$ to produce the patched state $h^{(l)}$ (Line 10). To ensure a smooth transition and maintain global coherence, $\alpha_t$ follows a decay schedule described in equation \ref{}, gradually reducing the steering influence as the generation sequence $t$ progresses toward the target length $N$. $h^{(l)}$ is injected into the model at layer $L$ via a hook mechanism, replacing the original activations to continue the forward pass, as is showcased in Line 11. $P_{\theta}$ then computes the next token distribution $x_t$ using outputs from the last hidden layer propagated with $h^{(l)}$ and sample the next token, building the final output sequence $X_t$ autoregressively during generation.





==> Texts/texts_old/s5_results_old.tex <==

\begin{table*}[ht]
    \centering
    \small 
    \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{4pt} 
    \scalebox{0.7}{
    \begin{tabularx}{25cm}{
        >{\centering\arraybackslash}p{2.5cm} % Model Name
        >{\centering\arraybackslash}p{2.5cm} % Method
        >{\centering\arraybackslash}p{1.5cm} % AB
        >{\centering\arraybackslash}p{1.3cm}
        >{\centering\arraybackslash}p{1.3cm}
        >{\centering\arraybackslash}p{1.3cm}
        >{\centering\arraybackslash}p{1.5cm} % MA
        >{\centering\arraybackslash}p{1.3cm}
        >{\centering\arraybackslash}p{1.3cm}
        >{\centering\arraybackslash}p{1.3cm}
        >{\centering\arraybackslash}p{1.5cm} % MUNCH
        >{\centering\arraybackslash}p{1.3cm}
        >{\centering\arraybackslash}p{1.3cm}
        >{\centering\arraybackslash}p{1.3cm}
    }
    \toprule
    \multirow{2}{*}{\textbf{Model Name}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{AB}} & \multicolumn{4}{c}{\textbf{MA}} & \multicolumn{4}{c}{\textbf{MUNCH}} \\
    \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
    &  & Div. $\uparrow$ & Qual. $\uparrow$ & Clus. Linkage & \#Clus. & Div. $\uparrow$ & Qual. $\uparrow$ & Clus. Linkage & \#Clus. & Div. $\uparrow$ & Qual. $\uparrow$ & Clus. Linkage & \#Clus. \\
    \midrule

    % Llama
    \multirow{7}{*}{\parbox{2.2cm}{\texttt{Llama-3.1-}\\ \texttt{8B-instruct}}} 
    & Div Prompt  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Top-$k$ &  &  &  &  &  &  &  &  &  &  &  & \\
    & Top-$p$  &  &  &  &  &  &  &  &  &  &  &  & \\ 
    & Top-$\eta\sigma$  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Min-$p$  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Entropy  &  &  &  &  &  &  &  &  &  &  &  & \\
    & G2  &  &  &  &  &  &  &  &  &  &  &  & \\



    % \cmidrule(lr){2-5}
    % \noalign{\vskip 1pt} \cdashline{2-8} \noalign{\vskip 1pt}
    % & DivGuide (\textbf{Ours})  &  &  &  &  &  &  \\
    \noalign{\vskip 1pt}\midrule\noalign{\vskip 1pt}


    % Gemma
    \multirow{7}{*}{\texttt{Gemma2-9B-it}} 
    & Div Prompt  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Top-$k$ &  &  &  &  &  &  &  &  &  &  &  & \\
    & Top-$p$  &  &  &  &  &  &  &  &  &  &  &  & \\ 
    & Top-$\eta\sigma$  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Min-$p$  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Entropy  &  &  &  &  &  &  &  &  &  &  &  & \\
    & G2  &  &  &  &  &  &  &  &  &  &  &  & \\
    
    \noalign{\vskip 1pt}\midrule\noalign{\vskip 1pt}

    % Phi
    \multirow{7}{*}{\parbox{2.2cm}{\texttt{Phi-4-mini-}\\ \texttt{instruct}}} 
    & Div Prompt  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Top-$k$ &  &  &  &  &  &  &  &  &  &  &  & \\
    & Top-$p$  &  &  &  &  &  &  &  &  &  &  &  & \\ 
    & Top-$\eta\sigma$  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Min-$p$  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Entropy  &  &  &  &  &  &  &  &  &  &  &  & \\
    & G2  &  &  &  &  &  &  &  &  &  &  &  & \\
    
    \noalign{\vskip 1pt}\midrule\noalign{\vskip 1pt}
    % Mistral
    \multirow{7}{*}{\parbox{2.2cm}{\texttt{Mistral-7B-}\\ \texttt{instruct-v0.3}}} 
    & Div Prompt  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Top-$k$ &  &  &  &  &  &  &  &  &  &  &  & \\
    & Top-$p$  &  &  &  &  &  &  &  &  &  &  &  & \\ 
    & Top-$\eta\sigma$  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Min-$p$  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Entropy  &  &  &  &  &  &  &  &  &  &  &  & \\
    & G2  &  &  &  &  &  &  &  &  &  &  &  & \\

    \noalign{\vskip 1pt}\midrule\noalign{\vskip 1pt}
    % Qwen3 
    \multirow{7}{*}{\parbox{2.2cm}{\texttt{Qwen3-8B}}} 
    & Div Prompt  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Top-$k$ &  &  &  &  &  &  &  &  &  &  &  & \\
    & Top-$p$  &  &  &  &  &  &  &  &  &  &  &  & \\ 
    & Top-$\eta\sigma$  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Min-$p$  &  &  &  &  &  &  &  &  &  &  &  & \\
    & Entropy  &  &  &  &  &  &  &  &  &  &  &  & \\
    & G2  &  &  &  &  &  &  &  &  &  &  &  & \\


    \bottomrule
    \end{tabularx}}
    \caption{Diversity comparison between DivGuide and prompt-driven baselines on three datasets. AB, MA stands for AnaloBench \cite{analobench} and Meterphoric Analogy \cite{tong-etal-2024-metaphor} respectively. In addition to diversity comparison using pairwise embedding cosine distance, we also compare median perplexity across the models. }
    \label{tab:main_results}
\end{table*}


\section{Results}

Following the setup introduced in Section \ref{sec:exp_setup}, we run our experiments on five open source models using three datasets and report the results in Table \ref{tab:main_results}. The number of analogy sentence generation is set to be 10, and we compute the pairwise cosine distance among the generation embeddings as the indicator of generation diversity (Avg. div. column in Table \ref{tab:main_results}). We also report the median perplexity in addition to the average generation diversity (Med. ppl. column in Table \ref{tab:main_results}). We compare our results with the three prompt-driven baselines identified in Section \ref{sec:motivation}, including vanilla, diversity and logic prompts. Full prompts are included in Appendix \ref{}.
% adds a specific instruction that requires the model to be creative and diverse in analogy generation. Finally, we include the detailed instructions on the standard thinking procedure of analogy-generation that involves converting \texttt{context} into logic abstractions and attach the target domain into the logic skeleton. We include logic prompt as the third baseline in our comparison. 

We observe a consistent increase in generation diversity using DivGuide, with an average of \texttt{NUM} \% from all five models across three datasets, respectively. Notably for the three baselines, we find that providing the full analogy-making logic to the model is not yielding analogies in better quality both in terms of diversity and output coherence described in perplexity. Specifically, there is a inferiority when compared to the prompting strategy that merely encourages diversity, which is showcased in \texttt{model-name} on \texttt{ds-name}, as the diversity drops from \texttt{NUM} to \texttt{NUM}.


==> Texts/texts_old/s6_analysis_old.tex <==
\section{Analysis}
% where to patch on model layers
% when does patching start to take effect
% ablation on steering alpha
In this section, we provide a comprehensive analysis of DivGuide focusing on how the exchange of hidden states between the source model $M_{source}$ and guide model $M_{guide}$ influence the dynamics of hidden states, which gradually lead to the promotion of analogy-making diversity. In addition, we provide ablation studies across various setups to find the robustness frontier of our DivGuide framework. 


\subsection{Emergence of Analogy Diversity}

Following the manifold hypothesis within transformer circuits \cite{!} that observes intensive reasoning regions within the model, we employ a similar perspective to investigate the efficacy of our DivGuide framework through the lens of layer dynamics during model inference. Specifically, we capture the fluctuations of both diversity and coherence dynamics when patching the edited hidden states from DivGuide into different layer positions. To further justify the efficacy of DivGuide, we include a control group that patches random gaussian noise during generation and plot the results jointly in Figure \ref{fig:patch_validity}. We then construct a scatter plot modeling the interplay between diversity and coherence and identify the Pareto Frontier among the patched transformer layers. The scatter plot and the Pareto Frontier layers are shown in Figure \ref{fig:patch_pareto}.

Results on \texttt{Llama-3.1-8B-instruct} showcase a notable performance gain both in generation diversity and coherence when DivGuide edited hidden states are patched into the \textit{middle layers} of the model. This implies that when the model is instructed to generate analogies, these layers plays important roles in controlling the diversity and coherence of the output sentence. Our findings also echo with works that look into the hidden layers of LLMs on other reasoning tasks \cite{!}. 

% \paragraph{} \vspace{-2mm}
% \paragraph{} \vspace{-2mm}


% Subfigures
% \begin{figure*}
%      \centering
%      % --- First Subfigure ---
%      \begin{subfigure}[b]{0.6\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/fig5_pareto.jpg}
%          \caption{TBD.}
%          \label{fig:div_scatter}
%      \end{subfigure}
%      \hspace{2mm} % Adds horizontal space between images
%      % --- Second Subfigure ---
%      \begin{subfigure}[b]{0.25\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{Figures/fig5_validity.jpg}
%          \caption{TBD.}
%          \label{fig:sub2}
%      \end{subfigure}     
%      \label{fig:intra_div}
% \end{figure*}

\begin{figure}[ht]
    \begin{center}
    \includegraphics[width=\linewidth]{Figures/fig5_validity.jpg}
    \end{center}
    \vspace*{-2mm}
    \caption{Dynamics of edited hidden states at different layers for \texttt{Llama-3.1-8B-instruct}. Purple line records the patching dynamics of DivGuide, grey line is the patching dynamics of Gaussian noise. }
    \label{fig:patch_validity}
    \vspace*{-5mm}
\end{figure}


% \begin{figure*}[ht]
%     \begin{center}
%     \includegraphics[width=\linewidth]{Figures/fig5_pareto.jpg}
%     \end{center}
%     \vspace*{-2mm}
%     \caption{Scatter plot on the interplay between analogy generation diversity v.s. validity in \texttt{Llama-3.1-8B-instruct}. Colored dots are the Pareto frontier that achieves optimal generation diversity and validity. The results showcase a concentration of optimal diversity and validity between layer 16 to layer 22. }
%     \label{fig:patch_pareto}
%     \vspace*{-5mm}
% \end{figure*}


\subsection{Ablation Study}

\paragraph{Model Sizes.} \hspace{-2mm} 

\paragraph{Steering Weight and Generation Steps.} \hspace{-2mm} 



\begin{figure}[ht]
    \begin{center}
    \includegraphics[width=\linewidth]{Figures/fig6_ablation_combined.png}
    \end{center}
    \vspace*{-2mm}
    \caption{Ablation results of \texttt{Llama-3.1-8B-instruct} on steering alpha and number of warm-up generation steps in DivGuide framework. }
    \label{fig:ablation}
    \vspace*{-2mm}
\end{figure}







